Deep Relational Reasoning Graph Network for Arbitrary Shape Text Detection

Arbitrary shape text detection is a challenging task due to the high variety and complexity of scenes texts. In this paper, we propose a novel unified relational reasoning graph network for arbitrary shape text detection. In our method, an innovative local graph bridges a text proposal model via Convolutional Neural Network (CNN) and a deep relational reasoning network via Graph Convolutional Network (GCN), making our network end-to-end trainable. To be concrete, every text instance will be divided into a series of small rectangular components, and the geometry attributes (e.g., height, width, and orientation) of the small components will be estimated by our text proposal model. Given the geometry attributes, the local graph construction model can roughly establish linkages between different text components. For further reasoning and deducing the likelihood of linkages between the component and its neighbors, we adopt a graph-based network to perform deep relational reasoning on local graphs. Experiments on public available datasets demonstrate the state-of-the-art performance of our method.

==> 0-abstract.tex <==
\begin{abstract}
For example.

\newif\ifib
\ibtrue%\ibfalse%
\ifib
AHHHHHH
\else
BBBBBB
\fi
\end{abstract}

==> fig_result_MLT.tex <==
\begin{figure*}[htbp]
	\begin{center}%\centering
	\subfigure{
		\begin{minipage}[t]{0.33\linewidth}
			\centering
			\includegraphics[height=0.7\linewidth,width=0.98\linewidth]{figures/result/MLT/ts_img_00857}
			%\caption{fig1}
		\end{minipage}%
		\begin{minipage}[t]{0.33\linewidth}
			\centering
			\includegraphics[height=0.7\linewidth,width=0.98\linewidth]{figures/result/MLT/ts_img_00063}
			%\caption{fig2}
		\end{minipage}%
	    \begin{minipage}[t]{0.33\linewidth}
	    	\centering
	    	\includegraphics[height=0.7\linewidth,width=0.98\linewidth]{figures/result/MLT/ts_img_00087}
	    	%\caption{fig1}
	    \end{minipage}%
	}
	\subfigure{
		\begin{minipage}[t]{0.33\linewidth}
			\centering
			\includegraphics[height=0.7\linewidth,width=0.98\linewidth]{figures/result/MLT/ts_img_00330}
			%\caption{fig1}
		\end{minipage}%
		\begin{minipage}[t]{0.33\linewidth}
			\centering
			\includegraphics[height=0.7\linewidth,width=0.98\linewidth]{figures/result/MLT/ts_img_00228}
			%\caption{fig2}
		\end{minipage}%
		\begin{minipage}[t]{0.33\linewidth}
			\centering
			\includegraphics[height=0.7\linewidth,width=0.98\linewidth]{figures/result/MLT/ts_img_07035}
			%\caption{fig1}
		\end{minipage}%
	}
	\end{center}%
	\caption{ Detection examples of our model on ICDAR 2017 MLT.} %Green region means true positive and red region means false positive.}
	\label{fig:result_MLT}
\end{figure*}


==> tables/tbCTW1500.tex <==
\begin{table}[htbp]
	\begin{center}%\centering
	\renewcommand{\arraystretch}{1.3}
	\begin{tabular}{c||cccc}
		\toprule
		Methods& R& P & H\\
		\hline
		%CTD \cite{CTD} &65.2 &74.3 & 69.5 &-\\
		%\hline
		TextSnake \cite{TextSnake} &85.3 &67.9 & 75.6 \\
		%\hline
		CSE \cite{CVPR19_CSE} &76.1 &78.7 & 77.4\\
		%\hline
		LOMO*$ ^{\dagger} $ \cite{CVPR19_LOMO} &76.5 &85.7 & 80.8\\
		%\hline
		LSE$ ^{\dagger} $ \cite{CVPR19_LSA} &77.8 &82.7 & 80.1 \\
		%\hline
		ATRR$ ^{\dagger} $ \cite{CVPR19_ATRR} &80.2 &80.1 & 80.1 \\
		%\hline
		ICG \cite{SegLink++} &79.8 &82.8 & 81.3\\
		%\hline
		TextField \cite{TextField}&79.8 &83.0 & 81.4\\
		%\hline
		MSR$ ^{\dagger} $ \cite{MSR} &79.0 &84.1 & 81.5 \\
		%\hline
		PSENet-1s$ ^{\dagger} $  \cite{CVPR19_PSENet} &79.7 &84.8 & 82.2\\
		%\hline
		CRAFT \cite{CRAFT} &81.1 &86.0 &83.5\\
		%\hline
		TextDragon\cite{TextDragon} &82.8 &84.5 &83.6\\
		
		PSENet V2$ ^{\dagger} $\cite{PSENet_v2} &81.2 &\textbf{86.4} &83.7\\
		%\hline
		\hline
		\textbf{ours} &\textbf{83.05 }&85.73& \textbf{84.37}\\
		\bottomrule
	\end{tabular}
    \end{center}%
    \caption{ Results on CTW-1500. $^*$ denote the results based on multi-scale tests. $ ^{\dagger}$ indicates that the backbone network is not VGG16.} %, Where $^{recg}$ Means the Prediction is Combined with the Recognition Branch, $^*$ Means the Multi-scale Test is Performed and 
    \label{table:CTW1500}
\end{table}

==> tables/tbICDAR13.tex <==
\begin{table}[htbp]
	\begin{center}%\centering
	\renewcommand{\arraystretch}{1.3}
	\label{tbIC13}
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		Methods& R& P & F &FPS\\
		\hline
		RRPN \cite{RRPN} &72 &90 & 80 &-\\
		\hline
		Textboxes \cite{textboxes} &74 &88 & 81 &11\\
		\hline
		Textboxes++ \cite{textboxes++} &74 &88 & 81 &-\\
		\hline
		RRD \cite{RRD} &75 &88 & 81 &-\\
		\hline
		PixelLink \cite{PixelLink} &83.6 &86.4 & 84.5 &-\\
		\hline
		SegLink \cite{CTPN} &83.0 &87.7 & 85.3 &20.6\\
		\hline
		Lyu et al. \cite{corner}&79.4 &93.3 & 85.8 &10.4\\
		\hline
		DDR \cite{DDR} &81.0 &92.0 & 86.0 &1.1\\
		\hline
		CTPN \cite{CTPN} &83.0 &93.0 & 88.0 &7.1\\
		\hline
		MCN \cite{MCN} &87 &88 &88 &34\\
		\hline
		He et al. \cite{DDR_TIP} &\textbf{89} &\textbf{95} &\textbf{91} &-\\
		\hline
		Mask TextSpotter\cite{MaskTextSpotter} &88.1 &94.1 &\textbf{91.0} &4.6\\
		%\hline
		%Mask TextSpotter$^{recg}$\cite{MaskTextSpotter} &88.6 &\textbf{95.0} &\textbf{91.7} &4.6\\
\iffalse
		\hline
		\hline
		Textboxes$^*$  \cite{textboxes} &83 &89 & 86 &1.3\\
		\hline
		Lyu et al.$^*$ \cite{corner} \cite{textboxes++} &84.4 &92.0 & 88.0 &1\\
		\hline
		PixelLink$^*$ \cite{PixelLink} &87.5 &88.6 & 88.1 &-\\
		\hline
		Textboxes++$^*$ \cite{textboxes++} &86 &92 & 89 &-\\
		\hline
		RRD$^*$ \cite{RRD} &86 &92 & 89 &-\\
		\hline
		RRPN$^*$ \cite{RRPN} &88 &95 & 91 &-\\
\fi
		\hline
		\hline
		\textbf{ours} &\textbf{0}& 0& 0 &0\\
		\hline
	\end{tabular}
    \end{center}%
    \caption{Results on ICDAR2013.}%, Where $^{recg}$ Means the Prediction is Combined with the Recognition Branch, $^*$ Means the Multi-scale Test is Performed and 
\end{table}

==> tables/tbTD500.tex <==
\begin{table}[htbp]
	\begin{center}%\centering
	\renewcommand{\arraystretch}{1.3}
	\begin{tabular}{c||ccc}
		\toprule
		Methods& R& P & F\\
		\hline
		SegLink \cite{SegLink}  &70.0 &86.0 &77.0\\
		%\hline
		PixelLink \cite{PixelLink} &73.2 &83.0 & 77.8\\
		%\hline
		TextSnake \cite{TextSnake} &73.9 &83.2 &78.3\\
		%\hline
		%Border(DenseNet-121) \cite{ASTD} &77.4 &83.0 &80.1\\
		%\hline
		%ITN \cite{ITN} &72.3 &\textbf{90.3} &80.3\\
		%\hline
		%Lyu et al. \cite{corner} &76.2 &87.6 &81.5\\
		%\hline
		TextField \cite{TextField}&75.9 &87.4 & 81.3\\
		%\hline
		MSR$ ^{\dagger} $ \cite{MSR} &76.7 &87.4 &81.7 \\
		FTSN$ ^{\dagger} $ \cite{FTSN} &77.1 &87.6 &82.0\\
		%\hline
		LSE$ ^{\dagger} $ \cite{CVPR19_LSA} &81.7& 84.2 &82.9\\
		%\hline
		CRAFT \cite{CRAFT} &78.2 & \textbf{88.2} &82.9\\
		%\hline
		MCN \cite{MCN} &79 &88 &83\\
		%\hline
		IncepText$ ^{\dagger} $ \cite{IncepText} &79.0 &87.5 &83.0\\
		%\hline
		ATRR$ ^{\dagger} $ \cite{CVPR19_ATRR} &82.1 &85.2 & 83.6\\
		%\hline
		\hline
		%\textbf{HAM-ResNet-50} &77.66 & 85.12 & 81.22\\%whscore
		\textbf{ours} &\textbf{82.30} &88.05& \textbf{85.08}\\
		\hline
	\end{tabular}
    \end{center}%
    \caption{Results on MSRA-TD500. $ ^{\dagger}$ indicates that the backbone network is not VGG16.}
    \label{table:TD500}
\end{table}


==> tables/tbTotalText.tex <==
\begin{table}[htbp]
	\begin{center}%\centering
	\renewcommand{\arraystretch}{1.3}
	\begin{tabular}{c||ccccc}
		\toprule
		Methods& Precision& Recall & F-score \\
		\hline
		%Baseline \cite{TotaText_baseline} &78.0 &68.0 & 73.0\\
		%\hline
		%CTD \cite{CTD} &74.0 &71.0 & 73.0\\
		%\hline
		TextSnake \cite{TextSnake} &82.7 &74.5 & 78.4\\
		%\hline
		ATTR$ ^{\dagger} $  \cite{CVPR19_ATRR} &80.9  &76.2 & 78.5\\
		%\hline
		MSR$ ^{\dagger} $ \cite{MSR} &85.2  &73.0 & 78.6\\
		%\hline
		CSE \cite{CVPR19_CSE} &81.4 &79.7 & 80.2\\
		%\hline
		TextDragon \cite{TextDragon} &85.6 &75.7 & 80.3\\
		%\hline
		TextField \cite{TextField} &81.2 &79.9 & 80.6\\
		%\hline
		PSENet-1s$ ^{\dagger} $ \cite{CVPR19_PSENet} &84.02 &77.96 & 80.87\\
		%\hline
		ICG \cite{SegLink++} &82.1 &80.9 & 81.5 \\
		%\hline
		LOMO*$ ^{\dagger} $ \cite{CVPR19_LOMO}&87.6 &79.3 & 83.3\\
		%\hline
		CRAFT \cite{CRAFT} &87.6 &79.9 & 83.6\\
		%\hline
		PSENet V2$ ^{\dagger} $\cite{PSENet_v2} &\textbf{89.3} &81.0 &85.0\\
		%\hline
		\hline
		\textbf{ours} &86.54 & \textbf{84.93} & \textbf{85.73}\\
		\bottomrule
	\end{tabular}
    \end{center}%
    \caption{Results on Total-Text, $^*$ means the Multi-scale test is performed. $ ^{\dagger}$ indicates that the backbone network is not VGG16. }%, Where $^{recg}$ Means the Prediction is Combined with the Recognition Branch, $^*$ Means the Multi-scale Test is Performed and 
    \label{table:TotalText}
\end{table}
